Single scattering and effective medium description in multilayer cylindrical metamaterials: Application to graphene and metasurface coated cylinders

Coated and multicoated cylinder systems constitute an appealing metamaterial category, as they allow a very rich and highly tunable response, resulting from the interplay of the many different geometrical and material parameters involved. Here we derive and propose an effective medium approach for the detailed description and analysis of the electromagnetic wave propagation in such systems. In particular, we investigate infinitely-long multilayered cylinders with additional electric and magnetic surface conductivities at each interface. Our effective medium approach is based on the well known in the solid state physics community Coherent Potential Approximation (CPA) method, combined with a transfer matrix-based formulation for cylindrical waves. Employing this effective medium scheme, we investigate two realistic systems, one comprising of cylindrical tubes made of uniform tunable graphene sheets and one of cylinders/tubes formed of metasurfaces exhibiting both electric and magnetic sheet conductivities. Both systems show a rich palette of engineerable electromagnetic features, including tunable hyperbolic response, double negative response and epsilon-near-zero and mu-near-zero response regions.

==> 1_submit/cover_letter.tex <==
To Prof. Laurens Molenkamp 
Editor-in-Chief 
Physical Review B 
American Physical Society 
1 Research Road 
Ridge, NY 11961 
U. S. A. 

Subject: Submission of a manuscript to Physical Review B 

Heraklion, January xx, 2022. 

Dear Editor,

Please find enclosed the manuscript entitled “Single scattering and effective medium theory description for graphene and  metasurface coated cylindrical nanotubes” by Charalampos P. Mavidis, Anna C. Tasolamprou, Eleftherios N. Economou, Costas M. Soukoulis, and Maria Kafesaki that we wish to submit to Physical Review B  for publication as a regular article. 

In this work we present the investigation of the effective properties in systems of multilayered rods with graphene or a metasurface with both electric and magnetic response that prove to be particularly suitable for the achievement of a wide range of metamaterial properties.
We start our analysis with the derivation of the transfer matrix method for a single cylinder comprised of several co-centered cylindrical layers of arbitrary and a two-dimensional material and/or a metasurface at each interface. 
Based on this approach we derive the effective medium model for this system based on the Coherent Potential Approximation (CPA).
We analyze the response of ensembles of single and multilayered graphene-coated and metasurface-coated rods starting from the single cylinder's scattering properties and eigenmodes.
Starting from the investigation of the single cylinder’s scattering properties and resonances, we analyze the response of ensembles of single and multilayered rods by means of the Coherent Potential Approximation (CPA).
Calculating and analyzing the CPA effective parameters, we find that our systems exhibit a large variety of interesting metamaterial properties, including hyperbolic dispersion, epsilon-near-zero, mu-near-zero and negative refractive index response.
The electromagnetic response is also highly engineerable with multiple degrees of freedom. Namely, in principle, by properly selecting the number of layers, the materials, the radii  the metasurfaces at each interface and the filling ratio of the rods the derived
This work extends the model presented in our previously published work in Physical Review B 102, 155310 (2020) to include cylinders of several layers and allows the introduction of surface currents at each interface.

Thus, we believe that our work provides interesting information to scientists in the broader metamaterials and photonics communities and hope that our manuscript will be considered for publication in Physical Review B. As possible reviewers of our manuscript, we suggest several eminent scientists listed on the next page, all of whom have not been informed separately on our manuscript. 

The manuscript consists of the following xx files: 1 RevTex text file, and xx PNG figures. 
Please note that our manuscript is not under consideration elsewhere. We propose the manuscript for section Semiconductors II: surfaces, interfaces, microstructures, and related topics. 

On behalf of all coauthors, we thank you in advance for your time and assistance. 

Sincerely yours, 

C. Mavidis, PhD 

Institute of Electronic Structure and Lasers, FORTH, Heraklion, Greece
Department of Materials Science and Technology, University of Crete, Greece
E-Mail: mavidis@iesl.forth.gr
Phone: +30 2810 39 1917

==============================
List of proposed referees for manuscript "Single scattering and effective medium theory description for graphene and  metasurface coated cylindrical nanotubes" 
